waveSLAM: Empowering Accurate Indoor Mapping Using Off-the-Shelf Millimeter-wave Self-sensing

This paper presents the design, implementation and evaluation of waveSLAM, a low-cost mobile robot system that uses the millimetre wave (mmWave) communication devices to enhance the indoor mapping process targeting environments with reduced visibility or glass/mirror walls. A unique feature of waveSLAM is that it only leverages existing Commercial-Off-The-Shelf (COTS) hardware (Lidar and mmWave radios) that are mounted on mobile robots to improve the accurate indoor mapping achieved with optical sensors. The key intuition behind the waveSLAM design is that while the mobile robots moves freely, the mmWave radios can periodically exchange angle and distance estimates between themselves (self-sensing) by bouncing the signal from the environment, thus enabling accurate estimates of the target object/material surface. Our experiments verify that waveSLAM can archive cm-level accuracy with errors below 22 cm and 20deg in angle orientation which is compatible with Lidar when building indoor maps.

==> aux-files/joergcomments.tex <==
some comments on the draft you sent.

In the intro you have to explain why we do this. This is not new or
better than mmWave radar. In fact mmWave radar would work better. This
makes sense when you already have mmWave connectivity on board, and you
need multiple mmWave nodes on the robot for robust connectivity (given
the directionality of the antennas). So you get the FTM-to-self for
free. Now our contribution is to show that such a simple setup actually achieves accuracy that is usable. Please4 update the intro accordingly.

"in a centimeter-level (e.g., 2 cm) is needed such as finding" -> I
wouldn't talk about this since we don't achieve this.

II. That's the very basics, but for a working solution we'd then have to
clean the point clouds and determine the walls, given noisy input data.
Where is the data processing/map creation described, from Fig 3?

III. Most of these we don't address. Why is this here? This sounds more
like it should be shortened and part of the intro.

Fig7: what error is this? Average error? Over how many trials? What are
the errors bars/quantiles?

Fig 8: how could we get more data points? The mmWave map looks too
sparse. Is this a corridor? What about the other 2 missing walls?

People detection: with a distance of 2m this is primarily for collision
detection (not people counting or something similar). I'd motivate this.
Also, how do you know it's a person, not a chair or pillar?

Material detection: this is misleading, we're not classifying which
material it is. This seems to be just a location error for different
materials. But this would only depend on the reflection coefficient and
surface roughness, not the type of material. I think this should be
rewritten. Why is the wall so bad? Rough surface?

Best,
   Joerg



   Hi all,
I'd first highlight doing SLAM with just communication and sensing,
e.g., for cheap robots that don't have more fancy sensors, and then I'd
mention that they can also help as supplementary tool, but this is less
convincing since LIDAR, dedicated mmwave radar etc. will usually give
better performance. They can help in situations with visual obstruction
like smoke.

Also we need to explain why we have multiple mmWave transceivers on the
robot for communication. We had discussed the motivation and telling a
good story is critical for a convincing paper.

Many icons in Fig 6 are too small to easily identify. It looks like you
only have the mmwave assisted case, but from the figure it is not clear
how we improve over LIDAR in the first place. What is the story and
supporting graphs to use only mmWave?

What about glass? This is where our FTM could be better than LIDAR but I
don't see this in the graphs. Or is this in case 3? Where the glass is
is not clear. Can we add the LIDAR distance error to the graphs so we
can compare?

Fig 7 looks weird. Why would the distance change which materials give
high/low error, especially since those are not particularly high distances.

Best,
   Joerg

==> aux-files/legacyintro.tex <==
\section{Introduction}
\label{sec:intro}
%navigation, localization and tracking needs in indoor environments
%For the intro, write first a brief phrase per paragraph in form of bullet points. That would make easier to polish the story of the intro
Indoor navigation, localization, and tracing solutions are attracting increasing attention from the research community due to their wide applicability in different types of use cases such as smart homes, autonomous robots, human-robot interactions, and computer vision. Outdoor maps are publicly available from companies such as Google, Apple, or Microsoft. However, such solutions for indoor maps do not exist mainly due to privacy and regulatory reasons. Some proprietary indoor mapping solutions have been developed by some of the above-mentioned companies including Google Maps Indoor, HERE maps, and Apple indoor mapping and surveying mobile application that allows users to create indoor maps with their mobile phones. To this end, in the last decade, a lot of the attention of the research community was focused on the development of techniques to assist in the creation of a map of an unknown environment. Rather than relying completely on users to slowly discover the indoor environment with their mobile or sensors, a promising alternative is to use mobile robots to create indoor maps in a rapid manner. Persons of interest can be then localized and traced accurately within the map. 

Existing mobile robot solutions for creating indoor maps use optical sensors, such as Lidars~\cite{lidar}, RGB cameras~\cite{camera},~\cite{camera-1} or stereo cameras~\cite{camera-2} to produce very accurate indoor maps. However, optical sensors experience significant performance degradation in the presence of dust, fog, or smoke. Moreover, their use is also significantly restricted in indoor environments with glass/mirror walls or insufficient light. While airborne obscurants regularly occur in emergency situations (e.g., dense smoke for firefighting), the indoor offices in the business centers are usually separated by glass walls and poor illumination. Acoustic sensor-based mapping and contact tracing approaches, such as ultrasonic~\cite{ultrasonic} and microphones~\cite{jade},~\cite{BatMapper}, are resistant to lighting dynamics, but they either have very limited sensing range or become ineffective in noisy environments. The demand for creating an indoor map in the above challenging situations motivates us to consider Integrated Communication and Sensing (ICAS) of millimeter wave (mmWave) WLAN which has recently emerged as one of the main innovations of the next generation of wireless communications. The use of higher frequency bands from mmWave, wider bandwidth, and denser distribution of massive antenna arrays in future 6G systems will enable the integration of wireless signal sensing and communication in a single system to mutually enhance each other. On the one hand, the communications system as a whole can serve as a sensor. It can explore radio wave transmission, reflection, and scattering to sense and better understand the physical world, providing a broad range of new services. On the other hand, the capabilities of high-accuracy localization, imaging, and environment reconstruction obtained from sensing could help improve communication performance such as more accurate beamforming, faster beam failure recovery, and less overhead to track the channel state information (CSI).

%WiFi sensing
The WLAN sensing technology in general uses WiFi signals to perform environmental sensing, by using the existing WiFi infrastructure and WiFi signals in indoor environments. WiFi signals can penetrate and reflect the objects of different materials during their propagation. As a result, the station (STA) or access point (AP) can process the received WiFi signals and sense the surrounding indoor environment, detecting obstacles and target movements. In general, we can classify WLAN sensing into two main categories, namely the received signal strength indicator (RSSI) and channel state information. The RSSI has been widely used in the early attempts of WLAN sensing~\cite{rssi},~\cite{rssi_csi} where based on the measured received signal strength at the receiver, different fingerprinting and geometric methods can be applied. For example, RSSI patterns at different locations can be used as fingerprints for localization. Different from RSSI, CSI provides finer-grained wireless channel information at the physical layer, which is thus considered an alternative solution for accurate sensing~\cite{csi_survey}. Channel amplitude and phase information over different subcarriers are presented in the CSI which provides the capability to discriminate multi-path characteristics. For instance, by processing the spatial, frequency, and time domain CSI at multiple antennas we can extract detailed multi-path parameters such as angle-of-arrival (AoA) and time-of-flight (ToF).

%mmWave
In addition to the sub-6 GHz WLANs, the IEEE 802.11ad amendment operates at 60 GHz with a bandwidth of 2.16 GHz to deliver data rates of up to 4.6 Gbit/s, and its recently standardized successor 802.11ay can reach up to 100 Gb/s through multiple in/multiple out transmissions (MIMO), higher order modulation schemes, and channel bonding. To achieve larger link distances, mmWave devices use directional antenna arrays to focus the emitted energy towards the intended receiver, since the range of a single omnidirectional mmWave antenna element is extremely limited. A large number of elements in directional mmWave phased antenna arrays enables a very accurate estimation of the angle of the signal propagation, and the high temporal resolution from the multi-GHz bandwidth provides excellent ranging accuracy. These characteristics make mmWave technology an ideal candidate to design highly accurate indoor mapping systems. 

An indoor mapping system can estimate the Angle of Arrival and Time of Flight of the path between an AP and a client to: \emph{i)}~create a map of the unknown environment and \emph{ii)}~localize a person of interest. In case this path is a direct Line of Sight (LOS) with a single reflection, the angle and range information from AoA and ToF will lead to an accurate estimate of a point in the indoor map. However, if the path to the client is Non-Line of Sight (NLOS) via one or more reflections, both angle and range information correspond to the reflection, which is usually far from the actual client position. This can either occur when \emph{1)}~only a reflected path exists, \emph{2)}~the reflected path is much stronger than the LOS path since the phased array antenna is steered towards the reflection, \emph{3)}~or the device orientation is such that the aperture of the antenna cannot capture the LOS path, e.g., when the client is directly pointing towards a wall. Thus, mmWave position estimates are either very accurate or have a high error.

To this extent, in this work, we start with a description of the fundamentals of mmWave sensing and relevant use cases in Sec.~\ref{sec:fundamentals} and Sec.~\ref{sec:usecase}. Next, we scope the work around Simultaneous Localization And Mapping (SLAM) and contact tracing where in Sec.~\ref{sec:solution} we present our solution. The prototype design and implementation that uses mmWave sensing to produce an indoor map where persons of interest can be localized is described in Sec.~\ref{sec:prototype}. We experimentally evaluate our solution in Sec.~\ref{sec:experimental} and elaborate on the challenges of applying mmWave sensing for SLAM and person localization in Sec.~\ref{sec:challenges}. Finally, we conclude this work in Sec~\ref{sec:conclusion}.
%IN THSI WORK WHAT WE DO

%Introduce the work, talk about the importance of ISAC, ISAC and WiFi and the applicability it will have in the nextG use cases. 

%Talk about use cases and how they are executed today with sensors.

%In today applicaitons that this is done with sensors hoever with the rise of 6G networks joint communicaiton and sesnisng has the potental to enable this precise accuratcy for tracing localization and navigation. 

%talk about joint communicaiton and sensing and metnion that In our work, we focus on mm-wave sensing using FTM and AoA, which we will often refer to as sensing.


%Accurate indoor localization is an enabling technology, with applications ranging from asset management and inventory tracking to assembly control for a variety of different industries. Within the research community, the mobile robotics domain plays an important role with a vast and continuously growing body of contributions. Popular localization sensors employed on-board robots include cameras [16], ultrasound sensors [8], laser range finders [17] and even infrared sensors [2], and are used independently or in combination with fixed landmark beacons [3]. Although such systems are proven accurate and efficient, their great disadvantage lies in the requirement for line-of-sight (LOS).

%In the introduction, we talk about ISAC and WiFi, nextG of wireless systems and then we  explain why our system uses mmWave bands and not sub-6GHz bands. Basically, mmWave enables a much more fine-grained ToF and AoA, therefore mmWave also enables accurate mapping as well. This has to be discussed in the motivation as well.

%most importantly, we need to describe clearly the challenge: which is the problem we solve? Just saying we do ISAC is too high level, we need to say that that's the umbrella and then delve into the specifics (i.e., we target SLAM "with" ISAC context plus to realize this we need to overcome this and that challenge). We need to list these and then frame it nicely. No need those to be new challenges, for example spatial abiguity is not, but if framed in the context of SLAM and ISAC then is there and we show we can solve it.

==> aux-files/structure.tex <==
%Suggested TOC (9 oages)

%Introduction (1.pg):
%Literature review on how and where can we use this new techniques,
%scenarios with fog, lights (industry), crystal...
%WE MAY NEED A FIGURE HERE
%Assistance as navigation for accuracy enhancement?
%check literature of use cases of mmwave
%End the section motivating the use case we present
%Here we talk about mmwave on Wifi and cellular and all the advantages it has. We talk about navigation, indoor mapping and localization solutions existing in literature.    Then we introduce the possibility of using mmwave as assistance for navigation/localization, and highlight it comes for free in cheap hardware.
%Briefly explain the new concepts introduced in the last ammendments and explain that we are using that to do an implementation on real hardware to test the performance.
%Last, explain the content of each section

%Principles of mmWave localization (1pg with fig) 2
%We explain the main contributions of 802.11az
%Here explain the FTM, consisting on AoA/AoD ISTA-RSTA and the TOF. 


%System overview (0.5 pag + fig) 3.75
%here we present the blocks of the solution. 
%mmwave
%mobile robot
%how to get the information and how to process it to reach the use case presented in previous section.
%Be as general as possible
%UPDATE THE FIG (PABLO)

%Prototype (1.5 pag + fig) 5.5
%present the hardware and software we have for
%robot
%mmwave
%the scripts used to collect data, parse and elaborate map.

%Device limitations (Here we explain the implementation limitation like tof and ftm error), as well as device gets tired
%HERE WE HAVE THE 2 FIGURES OF FTM AND AOA(tof left aoa right)
%(explain problems for ex with data collection???)

%Experimental validation (2 with figures hector full page big and material small over the column) 7.5
%Here we have to show that our solution works:
%Combined maps mmwave with lidar due to lack of points?
%HECTORMAP MMWAVE FIGURE (BIG)
%show test on materials and explain the accuracy depending the roghness, since mmwave wavelenght small
%MATERIAL GRAPH
%test on detecting moving objects? People test i did for madrid?


%Related work (0.5 pag) 8
%on mapping using communications (even sub6 is ok).
%See through smoke is most similar one
%other map solutions or other mmwave applications of FTM may work.

%Conclusions and challenges? (0.5) 8.5
%Very early stage but huge potential
%Highlight it comes for free, very cheap and efficient
%Same as commag challenges for FTM
%Accuracy of odometry, integration with ROS?

%ref (20/30) (0.5) 9 total pages


==> aux-files/todo.tex <==
section1- Milan address comments from Claudio(MILAN)
section2- some comments left from Claudio- Pablo and Alejandro need to discuss how to address( ALEJANDRO)
section3- fig 2,3  update (MIlan)
section4- explain the corridors and figure match and fix the fig 3. Remove the blue  area and make sure to change cases with areas and match them with corridors(PABLO). check after section V.A and the whole paper to be cohirent in using the corridor numbers and areas.
section 5- change the figure of the maps according to what Milan and Pablo agree (PABLO)


substitute figure 5 with the current description only two curves one lidar and one waveSLAM (1m dist., best )


1) principles last para on sec 3 and test on experimental

==> extension.tex <==
1) experimental section extension
-Grab the dog

Identifica las áreas que requieren mayor desarrollo: Analiza tu paper de conferencia y determina las secciones que necesitan una expansión más sustancial. Pueden incluir la introducción, la revisión de la literatura, los métodos, los resultados o la discusión.

--REMAKE INTRO 
--REMAKE RESULTS
--ADD DISCUSION ABOUT STAND ALONE OR NOT AND DEVICES
--2ND order reflections with MD-track check other signal and azimuths
--Elevation for measurement rela


Añade más detalles y resultados: Expande la sección de métodos proporcionando más información sobre los procedimientos experimentales, el diseño del estudio y las configuraciones utilizadas. Agrega más resultados, análisis y gráficos para respaldar tus afirmaciones.

Realiza experimentos adicionales: Si es posible, lleva a cabo nuevos experimentos para complementar los resultados presentados en tu paper de conferencia. Estos experimentos adicionales pueden fortalecer tus conclusiones y proporcionar una base más sólida para tu trabajo.

--DESIGN NEW PROTOTYPE ON BETTER HARDWARE NEW IMAGE NEW STRUCTURE
--DOG SMALL ROOMS DIFFERENT PROTOTYPE
--EXTENSION FOR ROS2?



Amplía la discusión: Elabora más en la discusión de los resultados y su relevancia en el contexto más amplio de la investigación. Considera las implicaciones y limitaciones de tu estudio, así como las posibles direcciones futuras de investigación.

Revisa y edita: Revisa cuidadosamente todo el artículo, prestando atención a la coherencia, la claridad y la estructura general. Asegúrate de que todas las secciones estén bien conectadas y de que el estilo de escritura sea apropiado para una revista académica.

Asegúrate de cumplir con los requisitos de la revista: Investiga las pautas de publicación de la revista a la que deseas enviar tu artículo ampliado. Asegúrate de seguir todas las directrices de formato y estructura, y ajusta el contenido según sea necesario.




----material type detection

---include absorbing in extensions

==> tocextension.tex <==
TOC EXTENSION

1.Introduction =
2.Principles =
3.waveSLAM =
3-4-Lidar or mmWave activation?  source selection? Algorithm to select if use one or both. Scheduling Communications and Sensing? 
4.Prototype =
5.Experimental
--waveslam capabilities
--testbed and data collection
--grid map accuracy
NEW: Material detection
NEW: People detection? Not sure reflections on people

6.Related work
7.Discussion updates?
8.Conclusion
